ECMAScript -- The journey of a programming language from an idea to a standard

A significant portion of the web is powered by ECMAScript. As a web technology, it is ubiquitous and available on most platforms natively or through a web browser. ECMAScript is the dominant language of the web, but at the same time, it was not designed as such. The story of ECMAScript is a story of the impact of standardization on the popularity of technology. Simultaneously, the story shows how external pressures can shape a programming language and how politics can mar the evolution of a standard. In this article, we will go through the movements that led to the dominant position of ECMAScript, evaluate the factors leading to it, and consider its evolution using the Futures Triangle framework and the theory of standards wars.

==> xxx-03-case-web-browsers.tex <==
Meta: The idea of this section is to provide an overview of web standardization and how it works. Simultaneously we explain the web as a platform for those that don't know it well. The point is to show how the need for standardization emerged from the community, how the standards bodies were created out of necessity, and how vibrant open source culture is now feeding back to the standards. The process isn't without its problems and it's good to highlight the challenges. The worst case is that you break the web if you make a mistake on a standard level.

Meta: In terms of modeling, this is perhaps a mixture of push (browser vendors) and pull (community innovation)

\cite{bernerslee1992}

\subsection{Web browsers}

Meta: This should contain brief history of the browsers

Both hypertext and information retrieval and access systems existed before the web was invented \cite{bernerslee1992}. \href{http://info.cern.ch/hypertext/WWW/TheProject.html}{World Wide Web} (www) combined the ideas within a single system. The web allows information retrieval and search through hyperlinks. Websites can consist of data indices and individual pages that may either exist in a file system or be completely virtual (see also Server Side Rendering (SSR)). Later on the technology enabled the emergence of search engines that crawl the web using so-called spiders.

\subsection{DOM}

\todo{Explain the DOM and how the standardization effort works (W3C + WHATWG + related history)}

\todo{Find a couple of concrete examples where pressure from open source has shaped the standardization effort}

\begin{itemize}
    \item "...a platform- and language-neutral interface that allows programs and scripts to dynamically access and update the content, structure and style of documents" \cite{wood1998}
    \item "Before DOM, every browser, editor, and transformation engine handled things their own way. With DOM, you can write scripts that will work in of different browsers and editors" \cite{phillips1998}
    \item Specifically, the DOM provides a programmatic API for interacting with the DOM structure
    \item When people speak of using the platform in the web context, most likely they mean the DOM
    \item Since the early days, many abstractions showed up
\end{itemize}

\cite{halpin2017crisis}
\cite{gibbinsweb}

“Living standard”: A new way of making standards? \cite{tabares2021html5}

\subsection{Browser wars}

\todo{Browser wars section from own lecture but with standard bits and triangles added.}

\subsection{What to learn}

==> xxx-04-javascript-and-jscript.tex <==
So-called browser wars provide a background for the next era of JavaScript. In 1996, Netscape held majority of the market \cite{sebenius2002} and at the same time Microsoft became aware of the threat it represents to the hegemony of its Windows desktop operating system. The threat had to do with the fact that Netscape considered its browser combined with servers a new type of distributed operating system rather than a single application \cite{severance2012javascript}. The realization that this new movement could displace Microsoft, motivated the development of Internet Explorer and also led to an alternative implementation of JavaScript called JScript \cite{wirfs2020javascript}.

% Microsoft was successful in its market entry and by 2002, it had gained most of the browser market share as seen in the Figure \ref{fig:browser-wars}. The shift in the market also had implications for JavaScript which we will see in the following sections.

% As Sun and Netscape announced JavaScript, the same week Microsoft announced its plans for making a version of Visual Basic a standard for creating www based applications for their competing browser Internet Explorer. Microsoft published a beta version of Internet Explorer 3.0 in May 1996 that included support for JavaScript in addition to Visual Basic Script (VBS) through what they called ActiveX Script. The idea was to allow plugging in any scripting language to allow the creation of interactive webpages through linking of ActiveX controls, Java applets, and other comparable technologies. \cite{wirfs2020javascript}

% TODO: Explain the background of the era and bring up ideas like browser wars (this can use the marketshare image). Doing this provides a context for the following.

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[scale=0.17]{browser_wars.png}
    \label{fig:browser-wars}
    \caption{\href{https://commons.wikimedia.org/w/index.php?curid=1128061}{By Wereon - Own work based on: Browser Wars.png}, CC BY-SA 3.0}
\end{figure}
\end{comment}

\subsection{JScript - a competitor appears}

% find another source for JScript?

To maintain feature parity with Netscape Navigator, Microsoft developed an interpreter called JScript for the language \cite{wirfs2020javascript}. Microsoft also implemented a solution called Visual Basic Script (VBScript) to built on top of their own technology. Having to support JavaScript was an unhappy but a necessary compromise to gain market share.

Given there was no official specification for JavaScript, Microsoft was forced to reverse engineer its implementation based on what Netscape did in order to remain competitive \cite{wirfs2020javascript}. Until a standard could emerge, the specification lived in Netscape's implementation of the language which at the time was not open source and available to study.

% On Microsoft side, Robert Welland started working on JScript in October 1995. His earlier experience included NewtonScript inspired by Self during his work at Apple so there was common background in terms of language design. Initially he was given the task of porting Visual Basic to the browser but he understood fast that it was too complicated to integrated with the browser's object model. He saw the initial JavaScript betas and implemented an early interpreter for the language. Combined with a language parser from the tools department of Microsoft and a gargabe collector from Patrick Dussud, the foundation for JScript had been built. \cite{wirfs2020javascript}

% Internally it was not clear if Internet Explorer should support JavaScript or if they should focus on Visual Basic. Given the target of the Internet Explorer team was to be compatible with Netscape Navigator 3, that forced Microsoft to add support even if they were not too happy about it. The compromise was to support both JavaScript and VBS for scripting. \cite{wirfs2020javascript}

% \subsection{Active Scripting}

% One of the interesting offshoots of the development was an embeddable scripting system called Active Scripting (AS). Active Scripting included support for both JavaScript and VBS and provided server-side scripting technology for Microsoft's Active Server Pages offering. One of the important parts of AS was a script debugger, a component missing from Netscape's offering. The hope was that the feature would draw developers to Microsoft side. Furthermore, to remain competitive, Microsoft put heavy effort to sustain compatibility with Netscape by testing their implementation against Netscape through thousands of websites. Any difference led to a reverse engineering effort to figure out what was different and subsequently allowd to match behavior across the browsers. \cite{wirfs2020javascript}

% \subsection{The cost of missing standard}

% The lack of language specification was a continuous source of consternation for the developers at Microsoft and as a result Thomas Reardon, the leader of Internet Explorer 3 effort, chided his counterparts at Netscape for a lack of standardization in the space \cite{wirfs2020javascript}. The impact of the lack of a standard can be seen in the necessity of reverse engineering to remain competitive. Until a standard could emerge, the specification lived in Netscape's implementation of the language which at the time was not open source and available to study.

\subsection{Discussion}

JScript represents an answer to the early success of JavaScript. It was Microsoft's forced answer to the competitive pressure exerted by Netscape Communications and therefore the birth of JScript was caused by \textbf{push of the present}. In order to compete for the same userbase as Netscape, Microsoft was forced to follow their example and aim for compatibility so that the same websites would work in their Internet Explorer browser. The need for compatibility represents \textbf{weight of the past} as the JScript effort would not have made much sense otherwise for scripting the web. Scripting was an important part of the \textbf{pull of the future} as it was a shared vision between Microsoft and Netscape although Microsoft put effort to port their technologies, such as Visual Basic, to the web and likely would have preferred to lead there with technology instead of following.

Out of these factors, push of the present and weight of the past stand out. The vision for the future seems less important as in this early stage of the web history, Microsoft's reply seems reactive instead of proactive. It can also be said that the potential value of the web was not still well understood in 1996 although that happened a few years later in the form of the dotcom boom.

The key learning of the JScript case is that competition can force the need for standardization to emerge. As there was no official specification for JavaScript, Microsoft was forced to reverse engineer it and as it goes with reverse engineering efforts, it is rarely perfect. It is this pressure that led to the birth of the ECMAScript standard as we will discuss in the next section.

% \todo{Explain history briefly and lead to standardiation}

\begin{comment}
\begin{itemize}
    \item Developed by Brendan Eich in ten days at Netscape \cite{eich2008}
    \item "I am not proud, but I am happy that I chose Scheme-ish first-class functions and Self-ish (albeit singular) prototypes as the main ingredients. The Java influences, especially y2k Date bugs but also the primitive vs. object distinction (e.g., string vs. String), were unfortunate." \cite{eich2008}
    \item 2011 - 38.2\% of sites use JavaScript - W3Techs
    \item 2022 - 82.3\% of sites use JavaScript - W3Techs
\end{itemize}
\end{comment}

==> xxx-05-case-ecmascript-modules.tex <==
Meta: The idea of this section is to show how messy and organic the standardization process can be when the initial standard is missing a core feature and then the community begins to innovate in the space to find a solution.

\subsection{CommonJS}

Meta: It is good to consider the constraints and the background here.

\cite{obcena2010javascript}

\subsection{AMD and UMD}

\subsection{ES2015 modules}

Meta: Explain why ES2015 modules were needed (static analysis vs. CommonJS) and what are the problem spots. It is also worth discussing import() most likely as that was an extension added later. For import(), webpack provided an initial solution through a different type of syntax that achieved the same internally.

\todo{Mention what Node.js did with mjs}
\todo{Mention the influence of TypeScript}

\subsection{What to learn}

==> xxx-10-case-edge-computing.tex <==
\section{Case edge computing – standardization through competition}

Meta: Compared to others, this is a clear push case where a group of companies is trying to improve the technology landscape to increase their adoption. It would be easy to posit that as the market becomes more stable, this will shift to a pull model.

Meta: In this case, the angle is a little different as we approach the topic from a company perspective. There is still open source in play as the related players implement their solutions largely in open source but the incentives are different as they are looking to replace the incumbents (mainly Amazon) with a new approach for which standardization gives the leverage they need to create a bigger market for all. This is an example of commercial pressure combined with open source pushing for standardization on WHATWG/W3C level.

\subsection{Edge computing}

\todo{Explain the term and why it's a relevant topic now for the web}

\subsection{WinterCG – Runtimes community group}

\todo{Explain how several smaller companies got together to create a market + to challenge the hegemony of Amazon}

% https://wintercg.org/

\subsection{What to learn}
